Comparing the Structures and Characteristics of Different Game Social Networks -- The Steam Case

In most games, social connections are an essential part of the gaming experience. Players connect in communities inside or around games and form friendships, which can be translated into other games or even in the real world. Recent research has investigated social phenomena within the player social network of several multiplayer games, yet we still know very little about how these networks are shaped and formed. Specifically, we are unaware of how the game type and its mechanics are related to its community structure and how those structures vary in different games. This paper presents an initial analysis of Steam users and how friendships on Steam are formed around 200 games. We examine the friendship graphs of these 200 games by dividing them into clusters to compare their network properties and their specific characteristics (e.g., genre, game elements, and mechanics). We found how the Steam user-defined tags better characterized the clusters than the game genre, suggesting that how players perceive and use the game also reflects how they connect in the community. Moreover, team-based games are associated with more cohesive and clustered networks than games with a stronger single-player focus, supporting the idea that playing together in teams more likely produces social capital (i.e., Steam friendships).

==> notes.tex <==
~\cite{perry2018online}
In support of recent perspectives arguing for positive benefits of
gaming, our findings highlight the role of establishing and maintaining social relationships with other players in building social
capital, as well as the type of engagement with the game that such
relationships facilitate. Overall, our study provides initial support
for two propositions from the People-Game-Play model (Johnson
et al., 2013): that individual and game characteristics impact
wellbeing by affecting the type of engagement with the game; and
that a harmonious type of engagement is the most important
determinant of positive wellbeing outcomes.

~\cite{fang2014competition}
both outside friends and inside friends will influence players’
payment willingness positively in social games. This finding
confirms the social influence theory in social gaming context
Second, we surprisingly found inside friends have more influence power than outside friends.

~\cite{depping2018designing}
that social capital in games is strongly and positively related
to players’ psychological well-being
Surprisingly, cooperation was not predictive of social
capital - examples in which competition does not
seem to be detrimental to relationship formation. Cooperation might be important in early
relationship formation but grow less important as
relationships develop. Nonetheless, our findings challenge
the common wisdom that multiplayer games need to be
cooperative to facilitate relationship formation.

~\cite{mason2013friends}
Contradicting the anti-social stereotype of FPS players, our
respondents were strongly motivated by social factors. More
than 99.5\% of our respondents indicated that they played with
at least one online friend, and the typical number was 21 online friends (and 4 offline friends).7 Nearly 80\% preferred to
play socially, on a team, rather than individually as a “lone
wolf,” and most players felt a strong sense of group cohesiveness and coordination. Thus, friendships among Reach
players play an important role in choices of play style, game
engagement and investment.

~\cite{verheijen2019influence}
Results showed that playing a game competitively lowered friendship quality. Furthermore, the mode of play changed the participants' behavior during game play, with more positive, negative, and hierarchical behavior observed in the cooperative condition. Additionally, positive and prosocial behavior displayed during the gaming session predicted higher friendship quality afterwards.

~\cite{trepte2012social}
Overall, the data confirmed our assumption that gaming in clans may foster the gamers’ offline contacts to other clan members, and may thus provide them with additional social support.
previous qualitative studies have suggested that gamers may increase their social support, if games would provide them with opportunities to “wind down” (Ducheneaut et al., 2007, p. 163) and socialize rather than merely focusing on their progress within the game. This assumption is supported by our data: As soon as gamers go one step beyond mere competition and ambitions solely related to game-play and engage in any kind of game- or team-management, they seem to gain more social support in both settings, online as well as offline.

~\cite{eklund2015bridging}
All the informants combined different genres
of games and themselves put emphasis on digital games as social
facilitators, giving a context for friendships to form, whilst adding
continuity to relationships with family and friends, both close by
and geographically separated.
In peoples’ practices several social worlds meet and the boundary between online and offline becomes contingent of these links.
In short, it seems that the importance of offline connections for the
creation and sanctioning of norms has been overlooked in previous
research. Understanding each other, keeping the same time schedule, and valuing the same things outside the online space are factors that influence this social ordering. Research should therefore
further explore this link in order to improve our understanding
of online interaction. As the current results are limited to the sample group at hand, more comparative studies are called for.

~\cite{lee2015homophily}
we ask whether an online casual game player tends to be friends with other online casual game players who have similar game genre preferences [..]  The results suggest that there
might not be strong homophily and social influence processes operating among the game players in the sampled network.


~\cite{rosell2017esport}
It is possible to say that there are at least two types of eSports, these are the MOBA and the
first-person shooter ones. The most popular and widely played examples of these are, League
of Legends (by Riot Games) for the MOBAs and Counter Strike: Global Offence (by Valve
Games) for the first-person-shooters. These are easily identified with the competitive practice
involving high degree of skill that gaming as a sports practice requires; and, therefore, they
can be called eSports. They are team games which require a lot of concentration, precision,
team rapport and shooting skill, however, since the games are different, both for their rules
and their mission, the practices diverge slightly.
